PARSAC: Accelerating Robust Multi-Model Fitting with Parallel Sample Consensus

We present a real-time method for robust estimation of multiple instances of geometric models from noisy data. Geometric models such as vanishing points, planar homographies or fundamental matrices are essential for 3D scene analysis. Previous approaches discover distinct model instances in an iterative manner, thus limiting their potential for speedup via parallel computation. In contrast, our method detects all model instances independently and in parallel. A neural network segments the input data into clusters representing potential model instances by predicting multiple sets of sample and inlier weights. Using the predicted weights, we determine the model parameters for each potential instance separately in a RANSAC-like fashion. We train the neural network via task-specific loss functions, i.e. we do not require a ground-truth segmentation of the input data. As suitable training data for homography and fundamental matrix fitting is scarce, we additionally present two new synthetic datasets. We demonstrate state-of-the-art performance on these as well as multiple established datasets, with inference times as small as five milliseconds per image.

==> tables/results_ob.tex <==
\begin{table*}
\smaller
\setlength\tabcolsep{.33em}
\renewcommand{\arraystretch}{1.2} 
	\begin{center}
	\begin{tabular}{|c|cc|cc|cc|cc|cc|}
	\hline
	   &
	\multicolumn{6}{c|}{SU3~\cite{zhou2019learning}} &
        \multicolumn{2}{c|}{HOPE-F} &
        \multicolumn{2}{c|}{SMH}\\
        \hline
	\multicolumn{1}{|l|}{outlier weights} & 
	\multicolumn{2}{c|}{AUC @ $1\degree$} &
	\multicolumn{2}{c|}{AUC @ $3\degree$} &
	\multicolumn{2}{c|}{AUC @ $5\degree$} &
	\multicolumn{2}{c|}{ME} &
	\multicolumn{2}{c|}{ME} \\
	\hline
% https://wandb.ai/tnt/segsac_vp/runs/ld7sde4i
% https://wandb.ai/tnt/segsac_vp/runs/ux0crg9i
	{yes}             
	& $\mathbf{67.45} $ & $\scriptstyle \pm 0.09$
	  & $\mathbf{85.73} $ & $\scriptstyle \pm 0.08$ 
        & $\mathbf{90.21} $ & $\scriptstyle \pm 0.08$  
        & $\mathbf{14.97} $ & $\scriptstyle \pm 8.51$  
        & $\mathbf{20.50} $ & $\scriptstyle \pm 15.5$
        \\
	{no}             
	& $63.79 $ & $\scriptstyle \pm 0.09$
	  & $83.94 $ & $\scriptstyle \pm 0.05$ 
        & $88.97 $ & $\scriptstyle \pm 0.08$  
        & $16.26 $ & $\scriptstyle \pm 9.10$    
        & $ $ & $\scriptstyle \pm $    \\
  
	\hline
	\end{tabular}
    \end{center}
	\caption{
	\textbf{Manhattan-world VP estimation:} 
 Average AUC values (in \%, higher is better) and their standard deviations over five runs for vanishing point estimation on the SU3 and YUD datasets. We omit standard deviations for deterministic methods. Average run times are given in milliseconds.
}
	\label{tab:results_ob}
\end{table*}


